Privacy Attacks Against Biometric Models with Fewer Samples: Incorporating the Output of Multiple Models

Authentication systems are vulnerable to model inversion attacks where an adversary is able to approximate the inverse of a target machine learning model. Biometric models are a prime candidate for this type of attack. This is because inverting a biometric model allows the attacker to produce a realistic biometric input to spoof biometric authentication systems. One of the main constraints in conducting a successful model inversion attack is the amount of training data required. In this work, we focus on iris and facial biometric systems and propose a new technique that drastically reduces the amount of training data necessary. By leveraging the output of multiple models, we are able to conduct model inversion attacks with 1/10th the training set size of Ahmad and Fuller (IJCB 2020) for iris data and 1/1000th the training set size of Mai et al. (Pattern Analysis and Machine Intelligence 2019) for facial data. We denote our new attack technique as structured random with alignment loss. Our attacks are black-box, requiring no knowledge of the weights of the target neural network, only the dimension, and values of the output vector. To show the versatility of the alignment loss, we apply our attack framework to the task of membership inference (Shokri et al., IEEE S&P 2017) on biometric data. For the iris, membership inference attack against classification networks improves from 52% to 62% accuracy.

==> RelatedWork.tex <==
%!TEX root = main.tex


\section{Related work}
\label{sec:related work}

\knote{Why is related work here? Shouldn't we just merge it with the introduction?}


% For privacy attacks (see~\cite{yeom2018privacy}) there is one critical region during model training, occurring when the network is overfitting to the provided data.  This means that the model is performing in a distinguishable way with respect to test data.  Previous works have used regularization and dropout in their networks to reduce overfitting and reduce the efficacy of privacy attacks. As stated in~\cite{shokri2017membership} the diversity of the training dataset also plays a role in the effectiveness of privacy attacks, with diverse data yielding less accurate privacy attacks.\footnote{Looking ahead, we confirm this belief, showing that related models from the beginning or end of a training/untraining process are more useful to an attacker in our attacks.  See Section~\ref{sec:results} and Table~\ref{tab:most useful models} for more detail.}





